Boosting of Thoughts: Trial-and-Error Problem Solving with Large Language Models

The reasoning performance of Large Language Models (LLMs) on a wide range of problems critically relies on chain-of-thought prompting, which involves providing a few chain of thought demonstrations as exemplars in prompts. Recent work, e.g., Tree of Thoughts, has pointed out the importance of exploration and self-evaluation in reasoning step selection for complex problem solving. In this paper, we present Boosting of Thoughts (BoT), an automated prompting framework for problem solving with LLMs by iteratively exploring and self-evaluating many trees of thoughts in order to acquire an ensemble of trial-and-error reasoning experiences, which will serve as a new form of prompting to solve the complex problem. Starting from a simple prompt without requiring examples, BoT iteratively explores and evaluates a large collection of reasoning steps, and more importantly, uses error analysis obtained from the LLM on them to explicitly revise prompting, which in turn enhances reasoning step generation, until a final answer is attained. Our experiments with GPT-4 and Llama2 across extensive complex mathematical problems demonstrate that BoT consistently achieves higher or comparable problem-solving rates than other advanced prompting approaches.

==> GSM8KFail.tex <==


\begin{table}[t]
    \centering
    \tiny
    \caption{BoT's success reasoning process.}
    \begin{tabularx}{\textwidth}{|X|}
        \hline
        \multicolumn{1}{|c|}{\textbf{Experience obtained in Iteration 1}} \\
        \hline
        \#\#\#\#\#\#\#\# The 1-th Reasoning Chain with Comments \#\#\#\#\#\#\#\#

        Below is a reasoning chain containing reasoning steps presented in order:

        -----------------------------------

                Step 1: Firstly, we need to calculate the total distance James runs each time he sprints. Since he runs 60 meters each sprint, and he does this 3 times a week, we multiply 60 by 3.. Evaluate Score: 0.7

                Step 2: After calculating the total distance James runs each time he sprints, we need to calculate the total distance he runs in a week. Since he runs 3 times a week, we multiply the total distance he runs each time by 3.. Evaluate Score: 1.0
        
        -----------------------------------
        
         Analysis Report: The reasoning chain can complete the task and reach the target correctly by executing its reasoning steps. The reasoning chain is correct and logical, and it successfully solves the problem by calculating the total distance James runs in a week.
        
        Reasoning step 1.
        Analysis: This step is logically correct. It accurately interprets the problem by identifying the need to calculate the total distance James runs each time he sprints. However, the description is slightly misleading. James does not run 3 sprints 3 times a week, he runs 3 sprints each time, and this happens 3 times a week. The multiplication should be between the distance of each sprint and the number of sprints each time.
        Advice: The description should be revised to "Since he runs 60 meters each sprint, and he does this 3 times each time he runs, we multiply 60 by 3."
        Recommendation: The reasoning step is correct, but the description needs to be revised for clarity.
        
        Reasoning step 2.
        Analysis: This step is a logical inference from the previous step. It correctly calculates the total distance James runs in a week by multiplying the total distance he runs each time by the number of times he runs in a week.
        Advice: No revision needed.
        Recommendation: The reasoning step is correct and should be accepted.
        
        Confidence score: 0.9
        
        \#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#
        \\ 

        \hline
        \multicolumn{1}{|c|}{\textbf{Experience obtained in Iteration 2}} \\
        \hline

        \#\#\#\#\#\#\#\# The 2-th Reasoning Chain with Comments \#\#\#\#\#\#\#\#

        Below is a reasoning chain containing reasoning steps presented in order:

        -----------------------------------

                Step 1: Firstly, we need to calculate the total distance James runs each time he runs. Since he runs 60 meters each sprint, and he does this 3 times each time he runs, we multiply 60 by 3.. Evaluate Score: 1.0
        
        -----------------------------------
        
         Analysis Report: The given reasoning chain can partially complete the task and reach the target. However, it is incomplete as it stops after calculating the total distance James runs each time he runs. It does not continue to calculate the total distance James runs in a week.
        
        Reasoning step 1. 
        The first step correctly calculates the total distance James runs each time he runs. It logically infers from the problem that since James runs 60 meters each sprint, and he does this 3 times each time he runs, the total distance he runs each time is 60 * 3. This step is beneficial to the correct solution as it is a necessary calculation towards finding the total distance James runs in a week.
        
        Advice: The reasoning chain needs to be continued to include the calculation of the total distance James runs in a week. This can be done by multiplying the total distance James runs each time he runs (which was calculated in step 1) by the number of times he runs in a week.
        
        Recommendation: Accept reasoning step 1 as it correctly calculates the total distance James runs each time he runs. However, the reasoning chain needs to be continued to include the calculation of the total distance James runs in a week.
        
        Confidence score: 0.9
        
        
        \#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#\#
        \\ 

        \hline
        \multicolumn{1}{|c|}{\textbf{Experience obtained in Iteration 3}} \\
        \hline

        \#\#\#\#\#\#\#\# The 3-th Reasoning Chain with Comments \#\#\#\#\#\#\#\#
        Below is a reasoning chain containing reasoning steps presented in order:

        -----------------------------------

                Step 1: Identify the elements in the problem. James is running 3 sprints 3 times a week, with each sprint being 60 meters. We need to find the total distance he runs in a week.. Evaluate Score: 0.9

                Step 2: Calculate the total distance James runs in a single day. Since he runs 3 sprints each day and each sprint is 60 meters, the total distance in a single day would be 3 sprints * 60 meters/sprint = 180 meters. Evaluate Score: 0.9. Evaluate Score: 0.9

                Step 3: Now, calculate the total distance James runs in a week. Since he runs 3 times a week and each time he runs 180 meters, the total distance in a week would be 3 days/week * 180 meters/day = 540 meters.. Evaluate Score: 1.0
        
        -----------------------------------
        
         Analysis Report: The reasoning chain does complete the task and reach the target correctly. Each step logically follows from the previous one and contributes to the solution of the problem.
        
        Reasoning step 1. 
        The first step correctly identifies the elements of the problem and the task at hand. It correctly interprets the problem statement and sets up the basis for the next steps. 
        Advice: None.
        Recommendation: Accept this step as it correctly identifies the problem and what needs to be done.
        
        Reasoning step 2. 
        This step logically follows from the first step. It correctly calculates the total distance James runs in a single day by multiplying the number of sprints he runs by the distance of each sprint. This step is beneficial to the solution as it breaks down the problem into smaller, manageable parts. 
        Advice: None.
        Recommendation: Accept this step as it correctly calculates the daily running distance.
        
        Reasoning step 3. 
        This step is a logical inference from the previous step. It correctly calculates the total distance James runs in a week by multiplying the distance he runs each time by the number of times he runs in a week. This step is beneficial to the solution as it completes the calculation and provides the answer to the problem.
        Advice: None.
        Recommendation: Accept this step as it correctly calculates the weekly running distance.
        
        Confidence score: 1.0
        \\
        \hline
        \multicolumn{1}{|c|}{\textbf{Ignore the subsequent iterations as the correct reasoning chain has been obtained.}} \\
        \hline
    \end{tabularx}

    \label{tab: gsm8kexample1}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

